Guidelines for Implementing and Auditing Differentially Private Systems

Differential privacy is an information theoretic constraint on algorithms and code. It provides quantification of privacy leakage and formal privacy guarantees that are currently considered the gold standard in privacy protections. In this paper we provide an initial set of "best practices" for developing differentially private platforms, techniques for unit testing that are specific to differential privacy, guidelines for checking if differential privacy is being applied correctly in an application, and recommendations for parameter settings. The genesis of this paper was an initiative by Facebook and Social Science One to provide social science researchers with programmatic access to a URL-shares dataset. In order to maximize the utility of the data for research while protecting privacy, researchers should access the data through an interactive platform that supports differential privacy. The intention of this paper is to provide guidelines and recommendations that can generally be re-used in a wide variety of systems. For this reason, no specific platforms will be named, except for systems whose details and theory appear in academic papers.

==> application.tex <==

\subsection{How Data Preparation Impacts Privacy}

Standard definition DP assumes input is a single table.  In many settings, raw data is in fact much more complex (e.g., a relational database with multiple tables) and must be pre-processed into the form of a single table upon which DP computation will be performed.  

\mh{walk thru some examples of data processing with a simple example that roughly approximates SS1 data}
raw data is three tables: person, url, urlShareEvent
\begin{itemize}
    \item processed table is share table joined with others: effectively guarantee hides on sharing event.  one user could contribute many rows.  each user's effective epsilon is different.
    \item processed table is url with aggregation of shares. bad on both fronts: same privacy issues as first, but now DP could throw out a lot of data.
    \item processed table is like first one, but with truncation (cap user to 100 shares).
\end{itemize}

\mh{add some discussion of papers that consider this further.  Dan's no free lunch, my privateSQL paper, etc.}

is n known (should not be because of bad composition with other data). but if n is known, sensitivity doubles

how to get attribute domains

\mh{some discussion of how the initial set of URLs is curated?  this step was not DP, but is, at least in theory, public knowledge}

\subsection{The Facebook Dataset}\label{subsec:facebook}



==> design.tex <==
\begin{itemize}
    \item privacy module should be small
\end{itemize}

==> groupings.tex <==
\section{Groupings of Related Functions}
These are functions whose tests should be similar.

\textbf{All functions should also be tested on empty input (i.e. a selection of rows that yields the empty set)}

\subsection{Linear single number outputs:}
\begin{itemize}
    \item Count
    \item Count Distinct (gets distinct items then applies count?)
    \item Count Cast (what does it do?)
\end{itemize}

\subsection{Linear vector-valued outputs:}
\begin{itemize}
    \item Histogram
    \item Histogram 2d (what is the difference from histogram?)
    \item Contigency table
    \item Describe
    \item GroupBy
    \item Skewness, Kurtosis, depending on how implemented
    \item logloss
\end{itemize}

\subsection{Nonlinear single-number outputs}
\subsubsection{Order based single number mechanisms:}
\begin{itemize}
    \item Quantile
    \item Median
    \item Inter-Quartile Range
    \item Min
    \item Max
    \item GroupBy (Min,Max)
    \item Guess Bound
\end{itemize}


\subsubsection{Aggregation function single-number outputs}
\textbf{Should also be tested on empty and single row inputs}
\begin{itemize}
    \item Sum
    \item Mean
    \item Variance
    \item MAE
    \item MSE
    \item $R^2$
    \item Accuracy
    \item AUROC
    \item AUPR
    \item ROC
\end{itemize}

\subsection{Rational Function multi-number outputs}
\begin{itemize}
    \item Covariance Matrix
\end{itemize}


\subsection{Regressions}
\textbf{Should also be tested on empty and single row inputs, along with multi-row colinear inputs}
\begin{itemize}
    \item Linear regression
    \item Logistic regression
    \item Generalized Linear regression
    \item Generalized logistic regression
\end{itemize}

\subsection{Unknown (depends how implemented)}
\begin{itemize}
    \item FilterFeatures
    \item NICV
    \item CV
    \item PCA
    \item Latent Dirichlet Allocation
    \item KMeans
\end{itemize}

==> stability.tex <==
\cite{ebadistability}
